Test Scenario Generation for Context-Oriented Programs

Their highly adaptive nature and the combinatorial explosion of possible configurations makes testing context-oriented programs hard. We propose a methodology to automate the generation of test scenarios for developers of feature-based context-oriented programs. By using combinatorial interaction testing we generate a covering array from which a small but representative set of test scenarios can be inferred. By taking advantage of the explicit separation of contexts and features in such context-oriented programs, we can further rearrange the generated test scenarios to minimise the reconfiguration cost between subsequent scenarios. Finally, we explore how a previously generated test suite can be adapted incrementally when the system evolves to a new version. By validating these algorithms on a small use case, our initial results show that the proposed test generation approach is efficient and beneficial to developers to test and improve the design of context-oriented programs.

==> FBCOP-old.tex <==
%\section{Background}
% Background – part 1

\section{Feature-based context-oriented programming}
\label{sec:fbcop}

Unlike other COP languages, FBCOP makes an explicit distinction between how contexts (reifying particular situations sensed from the surrounding environment) and features (behavioural variations specific to certain contexts) are modelled and handled~\cite{Duhoux19ImplFBCOPL, Duhoux19SATToSE}. Taking inspiration from Hartmann and Trew's \emph{multiple product line feature model}~\cite{Hartmann08FeaturesContexts}, in FBCOP
contexts and features are modelled as two separate feature diagrams: a \emph{context variability model} describing the potential situations for which the system has a running variant and a \emph{feature model} describing the common functionalities and variability points of the system, specific to certain contexts.

Figure~\ref{fig:FBCOApproach} depicts the FBCOP architecture
showing its overall lo\-gic and models involved.
%As the picture suggests, 
The approach consists of four subsequent phases:
context activation, 
feature selection, feature activation and feature execution.

\begin{figure}[h]
  \centering
  \includegraphics[draft=false, width=\linewidth]{images/FBCOApproach}
  \caption{Overview of the different models and phases in a feature-based context-oriented program~\cite{Duhoux19ImplFBCOPL}.}
  \Description{}
  \label{fig:FBCOApproach}
\end{figure}

\paragraph{Context activation}
The set of all possible contexts is modelled as a feature diagram called \textit{context model}~\cite{Desmet07CODA, Hartmann08FeaturesContexts}.
This context model represents all different situations of the surrounding environment to which the system is able to adapt its behaviour.
In this model, each context can be selected or not. A selected context means that the context is active and describes a specific situation of the environment in which the system runs; a non-selected context is inactive and does not have an impact on the current behaviour of the system. 
During the first \textit{context activation} phase,
when a particular situation in the surrounding environment is sensed (resp. no longer sensed), the system attempts to activate (resp.  deactivate) it.
For that the system updates the current configuration of the context model, representing the current state of the surrounding environment, with the newly discovered context. It verifies if all hierarchical and cross-tree constraints of the model remain satisfied. If the new configuration is valid and satisfies all constraints, this new configuration is kept and the system proceeds to the second \emph{feature selection} phase. Otherwise, the system rolls back to the previous valid configuration of the context model and ignores the new context.

\paragraph{Feature activation}
Before explaining the \emph{feature selection} phase we explain the \emph{feature activation} phase which is very similar to the \emph{context activation} phase. Like the context model, the set of all possible behavioural variations is modelled as a feature diagram called \textit{feature model}.
A feature in this model represents a possible behavioural variation that can dynamically get activated depending on what contexts are currently active.
The feature diagram declares all possible hierarchical and cross-tree constraints between these features.
A particular configuration of the feature model describes the set of currently active features.
After the features get (un)selected in the second \emph{feature selection} phase, the system will try to activate selected and deactivate unselected features by instantiating another configuration of the feature model.
If after (de)activating this set of features the configuration is no longer valid, the feature model configuration rolls back to a previous valid state.

%Observe how Figure~\ref{fig:FBCOApproach} contains an extra node (depicted as a dashed rectangle) that combines the context and feature model in a single unified feature diagram. This is similar to how Hartmann and Trew combined both models~\cite{Hartmann08FeaturesContexts} and will come in handy further in this paper when calculating a covering array of scenarios consisting of relevant combinations of contexts and features. 

\paragraph{Feature selection}
As depicted in Figure~\ref{fig:FBCOApproach}, 
The context and feature model and their corresponding context and feature activation phases, are connected through a \textit{mapping model} in the \textit{feature selection} phase.
This is a crucial part of the approach, as
the mapping model describes how the system must be adapted by which features, depending on what contexts were sensed in the surrounding environment.
It is expressed as a conjunction of individual mappings, where each individual mapping is a \emph{N:N} relation from contexts to features. When all source contexts of such a mapping are active, the system will select the target features to activate and propagate this selection to the \emph{feature activation} phase.
Conversely, when one of the source contexts of an individual mapping becomes inactive, the target features of that individual mapping get unselected.

\paragraph{Feature execution}
Once all features have been activated in the \textit{feature activation} phase, during the \emph{feature execution} phase the system will adapt its behaviour with the newly (de)activated features to modify its behaviour. For this, the system will install or remove the code associated with these features in its running code to refine or change its observable behaviour. Since this phase is less relevant for this particular paper we voluntarily omit some details on this phase. For more information on how this is achieved and other implementation details, please consult this paper~\cite{Duhoux19ImplFBCOPL}.

\subsection{Case study} %[1p max]
\label{sec:case}
As a running example, we now describe a small FBCOP application that serves as case study throughout this paper.

The application consists of a \textit{messenger system}, allowing users to exchange messages, and is \textit{smart} in the sense that it can adapt or refine its behaviour depending on some contextual situations. A simplified version of the context, mapping and feature model of this system is depicted in Figure~\ref{fig:casestudy-models}.

\begin{figure*}[h]
  \centering
  \includegraphics[draft=false, width=\linewidth]{images/CaseStudyMessenger}
  \caption{Design of a prototype of our smart messenger system. The context model is on the left, the feature model on the right and the mapping model in between these two. We voluntarily omitted some mapping details for readability reasons.}
  \Description{}
  \label{fig:casestudy-models}
\end{figure*}

The main functionality of our smart messenger system is \emph{Sending} or \emph{Receiving} messages to and from other users. By default, we assume the messages are of type \emph{Text}, but depending on the context (\emph{Peripheral}, \emph{Connection}) the system can handle messages of another \emph{MessageType} as well.
E.g., if the device on which the application runs possesses a \emph{VideoCard} to improve its graphic performance and the system senses a \emph{Good} connection, the user can send or receive pictures (\emph{Photo}). When an \emph{AudioCard} is present as \emph{Peripheral}, conversation can happen via \emph{Vocal} messages.

A conversation can take place between any two \emph{Friend}s. Each user is identified by its unique name (\emph{FriendName}). \emph{Teen} users may provide a \emph{ProfilePicture} in addition to their name. \emph{Adult} users can provide 
a textual \emph{Description} of themselves. Conversations can also be carried out between a \emph{Group} of friends, to which more friends can be added during conversation time.
To find and add friends, the system offers a \emph{Search} bar that \emph{Adult} users can use to look for a friend's name. For \emph{Teen} users, the only way to add friends is through a \emph{Match} system where the application suggests the teenager potential new friends that are connected to his known friends.
%, to encourage new encounters and friend\-ships with related teenagers.
\footnote{Every Teen user will always have minimum one friend as the only way to get access to the application is by invitation of a friend.}

%Whenever a new message is received, the user may receive a \emph{Notification} via an \emph{Alarm} or via a phone's \emph{Vibration} motor. What notification system is used can vary depending on the time of the day or the \emph{Noise} level of the environment. An alarm can only be used during \emph{Day} time and if the device is equipped with a \emph{SoundCard}. In case the 
%surrounding environment's \emph{Noise} level is too \emph{Loud}, the \emph{Notification} mode would be set to \emph{Vibration}, so that the alarm can be felt rather than heard. Finally, the notification system can be muted in order not to disturb the user when he is occupied such as during a meeting or at \emph{Night}. 

Whenever a user receives a new message, a \emph{Notification} may be given via a sound \emph{Alarm} or via the phone's \emph{Vibration} mode. What notification mode will be used depends on the \emph{User Availability} and on the \emph{Noise} level of the environment. Assuming the phone is equipped with an \emph{AudioCard}, an \emph{Alarm} can only be used when the ambient \emph{Noise} level is \emph{Normal} and the user is \emph{Available} (i.e., not in a meeting or other situation where the phone is muted). In case the ambient \emph{Noise} level is too \emph{Loud} or if the user is \emph{Occupied}, the \emph{Notification} mode would be set to \emph{Vibration}. Finally, the notification system can be muted when the ambient \emph{Noise} level is \emph{Quiet}, so as not to disturb the user, or when the user is \emph{Occupied}.

The \emph{Device} type may also affect the possible features of the smart messenger system. On a \emph{Smartphone} with smaller screen, the system uses a \emph{Minimalist} \emph{Layout} that restricts the information to \emph{Display} to the content and author of the current message being read. For a \emph{Device} like a \emph{Tablet} or \emph{Desktop} computer with larger screen and \emph{VideoCard}, a more \emph{Complete} \emph{Layout} can be used to reveal more information. Such a layout offers a user interface widget that lists all conversations on the left and another widget that exposes a selected conversation on the right. The system can also \emph{Display} a virtual \emph{Keyboard} on a \emph{Device} such as a \emph{Tablet} or a \emph{Smartphone} that does not have a physical keyboard. Finally, in order to reduce data consumption, the smart messenger offers the possibility to switch from \emph{Standard} to \emph{Light} \emph{Mode} depending on the \emph{Connection}. \emph{Light} mode may decrease the quality of the images or of conversation gadgets such as emojis.

Now that we have explained the main contexts and features of 
the system, we briefly revisit how they all work together in a FBCOP approach.
Assume an \emph{Adult} uses the smart messenger system on her \emph{Smartphone} which has an \emph{AudioCard} built in, is currently \emph{Available} for conversation, and that the ambient \emph{Noise} level in the surrounding environment is \emph{Normal}. Thanks to the declared mapping model, these contexts will trigger the activation and deployment of the following features in the messenger system: an \emph{Alarm} to notify the user of new messages received through a small buzzing sound, the ability to use \emph{Vocal} messages in addition to mere \emph{Text} messages, the ability to \emph{Search} for friends to add them to a group conversation, as well as the ability to add a detailed \emph{Description} to her user profile (thanks to the presence of the \emph{Adult} context). As she uses a \emph{Smartphone}, a \emph{Minimalist} layout and virtual \emph{Keyboard} will also be deployed in the system.


==> Future-work-old.tex <==
\section{Conclusion and Future Work}
\label{sec:conclusion}

This paper addressed the problem of generating test suites for programs written in a feature-based context-oriented programming language. Our first contribution was to reduce the problem to one of computing test suites for highly re-configurable systems with constraints. We then showed how to rearrange the test scenarios in such a test suite to minimize the number of context switches between each scenario. Finally, we explored an algorithm to incrementally augment existing test suites upon program evolution.

Validation of context oriented programs (whether feature-based or not) is at its infancy. There exists a wide range of possibilities to extend, improve upon, or complement the work presented in this paper. For example, we could improve Cohen's algorithm~\cite{cohen2008constructing} by exploiting the fact that our SAT formulas are produced from feature diagrams representing both a system's features and contexts. Exploiting such representation with algorithms such as those presented by Johansen~\cite{johansen2012algorithm} and Kowal~\cite{kowal2016explaining}  could help to pre-identify dead/core features or other anomalies that should be embedded in or rejected from each test scenario. Another possibility to achieve this objective would be to use Quantified Boolean Formula solvers~\cite{mauro2021anomaly}. 

Recent SAT solvers could also allow us to randomly compute valid configurations of SAT formulas. They have been shown to be efficient to estimate the t-wise coverage of various large size examples~\cite{PAPDC19,BLM20}. However, they have not yet been adapted to handle systems with constraints. 
%It would also be interesting to use recent sat-solvers that allows us to randomly compute valid configuration of SAT-Formula. In \cite{PAPDC19,BLM20}, they have been shown to be efficient to estimate the t-wise coverage of various large size examples. On the other hands, they are not yet adapted to handle systems with constraints. 

%We also think that 
The rearrangement process could also be extended by considering other objectives. In the spirit of Devroey et al.~\cite{DPCSLSH17}
%As an example, in the spirit of \cite{DPCSLSH17},
one could target rearrangements that prioritize those contexts that have been identified to be used frequently in deployed systems. We could also explore strategies that give more importance to some pre-defined high-frequency switches between contexts. Another possible extension is to consider new ways to generate the partial scenarios used in the augmentation procedure. 

Finally, the main objective of this paper being to pose the foundations of our new theory, the experimental section has been reduced to its minimum. So far, our prototype has been applied to a small academic case study only. The cost of creating a test suite for it and augmenting it has been reduced by more than half. In future work, we will investigate how its performance scales to industrial case studies. 

==> old-future <==


\authorcomment[idea]{PM}{If the new system includes too many new features and new constraints, and finding scenarios to fit the old test suite is impossible, there exists an alternative way to generate scenarios. At step 2, using the SAT solver, propagate Test case $t_k$ to new features and contexts. If there are still a feature and context left unassigned (which means that both the values True or False are compatible with the test case), then assign it to a different value that the scenario used in Test Case $t_{k-1}$). The created scenario can then be tried on the next $S$ Test cases. This kind of generation on the fly assures to find compatible scenarios for all test cases, if there is one, but will lose in diversity.}

\section{Future work}
\label{future-work}
That is, each test will generate two configurations. The algorithm keeps all resulting configuration that is satisfied and consider them to be part of the new test suite. If the configuration with the Boolean variable set to false is satisfied, then we have the guarantee that pairs from the origin test are still covered, but no more. If the configuration with the Boolean variable set to true is satisfied, then we not only keep the old pairs, but we also add pairs that cover the new feature/context.
\begin{itemize}
    \item We defined a specific re-ordering and distance between test cases, which is the number of switches of contexts between them. We could also explore other kind of re-ordering or prioritization, for example based on the probability a test case is likely to occur in real situations. We could also define other kinds of re-ordering where we try to encourage or discourage certain kinds of transition (e.g., try to maximize the number of transitions between the "Occupied" context and the "Available" context, because we want to test the robustness of our system against high-frequency variations in these contexts). The objective explored in this paper was "cost minimization", but other concepts could proposed for other objectives (more thorough testing ? ...).
    
    \item The SAT solver could be used more extensively to detect anomalies in the models (core and dead features). We already make a crude analysis of the core features, but other works already explored more optimal way to discover them \cite{johansen2012algorithm}. Integrating such discoveries with our methodology, or at least exploring some possible reuse, would be highly relevant.
    
    Feature model analysis could also be used to find these anomalies. This was already explored, for example by Mauro et al. \cite{mauro2021anomaly}.
    
    On the subject of further optimization, Cohen et al. already proposed some possible optimizations, also by exploiting further the possibilities offered by SAT solving \cite{cohen2008constructing}). We did not extensively the influence of these optimizations on the computation time to generate covering array for our kind of systems, as we do not really expect any surprising results,
    
    \item Validate this methodology to more diverse and industrial fb co systems. Unfortunately, we still do not possess this kind of fb co systems. The methodology is theoretically very scalable, as the size of the covering array grows logarithmically in the number of contexts and features, but more thorough studies on the scalability of the computation time could be done.
    
    \item The tool can create scenarios; can create the list of mandatory contexts/features. We also use the propagation functionality of modern SAT solvers as an optimization in Section \ref{}. However, we could also retrieve the information generated in this optimization to create a list of propagation inherent to the (de)activation of contexts or features. This list could be the starting point of new visualization tools. It would help the developer to improve the design of his application by providing another way to visualize the current interactions on his system, a tool who would aid him in his task of visualizing the consequences of all of the system constraints.
    For example, this tool would show a context model and you can click on contexts to highlight and (de)activate them, and it would in turn highlight all the (de)activation of contexts and features that are related to this action.
    
\end{itemize}

(- Tseitin transformation ?)



==> oldcit.tex <==
%%A feature model converted in such a way is a very constrained system, as %%each feature is present in at least one constraint, and all features are %%related one way or another through constraints. That is the first reason %%we need an algorithm that takes into account these constraints at its %%core. A greedy approach of a CIT sample generation technique that %%exploits calculations made by modern Boolean satisfiability (SAT) solvers %%to prune the search space of the CIT problem, thereby handling %%efficiently highly constrained systems, was first presented by Cohen et %%al. in 2008 \cite{cohen2008constructing}.

Generating a covering array for a feature model without considering the constraints between the features and trying to regenerate the test cases in violation with those constraints would perhaps work. However, in our system, not only are our models constrained by themselves, but the constraints are multi-layered and they create a network that spans both context and feature models through the mapping. If we generate a covering array for the contexts and another one for the features, or simply one for the features (as the code to be tested is directly related to the features), removing invalid configurations (and even valid configurations that do not match with valid configurations for the context model, because of the mapping and the constraints on the context model itself) to regenerate the covering array will be impossible in practice, due to the huge number of configurations concerned. These supplementary constraints on the feature model is the second main reason to our choice of algorithm, which will handle the context and the constraints it entails through SAT solving.

What follows is naturally to translate feature-based context-oriented systems in a form that suits the algorithm of Cohen. That is, a set of features with a number of variants for which a covering array will be generated, and a set of Clausal Normal Form (CNF) Boolean formulas which will be fed to the SAT solver. That is the process represented by the \textit{Model unification} module in Fig. \ref{fig:methodology-diagram}.

The first step we take is to reconcile features and contexts into a single unified feature diagram with a root node above both of these models, as seen in Fig. \ref{fig:FBCOApproach}. On a side note, this reconciliation is very straightforward, as these models were originally inspired by Hartmann et al. in \cite{Hartmann08FeaturesContexts}, where their context variability model and feature model were already connected and united by a root node above both of these models. \authorcomment[idea]{PM}{Is it the correct formulation ?}

Afterwards, as discussed previously, we can convert it to a set of features with the variants "activated" and "deactivated", or Boolean variables with the values "True" and "False" for clarity. Indeed, the constraints due to the feature modelling and the mapping are directly related to this set. Hence, the contexts and features will be used later in Boolean expressions as Boolean variables.

The relationships in the united feature diagram are then easily converted to their CNF form. Indeed, feature modelling was already formally translated to propositional logic \cite{czarnecki2007feature}, and propositional logic is directly translatable to CNF. On a side note, SAT solving and CIT was already proved to be efficient in handling feature diagrams \cite{johansen2011properties, johansen2012algorithm, mendonca2009sat}.

%\subsubsection{Simplification of the step 3} In the step 3 of the algorithm of Cohen, presented earlier, we need to find the new value $v_n$ that maximizes the number of pairs that will be covered by the new test case and that will not make this test case invalid. In our case, the number of possibilities $l_n$ is always 2 : a feature can either be activated or deactivated. Hence, if adding one of these two values to a valid partial configuration makes it invalid, then the other must be correct. This second value can then be directly added to the test case without any call to the SAT solver needed, which would avoid another portion of SAT calls. 

%With this simplification in mind, we now know that there are exactly $\left[M * S * (N)\right]$ calls to the SAT solver (with N the number of contexts and features), where S is in O(log(N)), which would mean that the number of SAT calls is in O($N * log(N))$.
%\authorcomment[idea]{PM}{I'm not sure of the utility of the previous paragraph and result. I just found it interesting, so I share the idea with you, but I think we can delete it.}
